RoCo: Dialectic Multi-Robot Collaboration with Large Language Models

We propose a novel approach to multi-robot collaboration that harnesses the power of pre-trained large language models (LLMs) for both high-level communication and low-level path planning. Robots are equipped with LLMs to discuss and collectively reason task strategies. They then generate sub-task plans and task space waypoint paths, which are used by a multi-arm motion planner to accelerate trajectory planning. We also provide feedback from the environment, such as collision checking, and prompt the LLM agents to improve their plan and waypoints in-context. For evaluation, we introduce RoCoBench, a 6-task benchmark covering a wide range of multi-robot collaboration scenarios, accompanied by a text-only dataset for agent representation and reasoning. We experimentally demonstrate the effectiveness of our approach -- it achieves high success rates across all tasks in RoCoBench and adapts to variations in task semantics. Our dialog setup offers high interpretability and flexibility -- in real world experiments, we show RoCo easily incorporates human-in-the-loop, where a user can communicate and collaborate with a robot agent to complete tasks together. See project website https://project-roco.github.io for videos and code.

==> text/introduction_v1.tex <==
\section{Introduction}
Multi-robot systems are intriguing for their promise of enhancing task productivity but face various challenges. First, an effective collaboration requires robots to split and allocate the work. This requires high-level understanding of a task, and consideration of each robot's capabilities such as reach range or payload. Another challenge lies in low-level motion planning - as the action space grows with the number of robots, finding collision-free motion plans becomes exponentially difficult. Finally, traditional multi-robot systems typically require task-specific engineering and hence compromises generalization: with much of the task structures pre-defined, a system is hard to adapt to new scenarios or variations in a task.  

In this work, we propose an approach using large language models (LLMs) to address these challenges, and demonstrate its effectiveness across a variety of multi-robot collaboration tasks. 

\textcolor{blue}{[LLM-enabled Robot Conversations]} 
First, we use a LLM to leverage LLMs for high-level task planning. We prompt an LLM to simulate chat among different robots, effectively letting the robots 'talk among themselves' and determine an action plan. This prompting method has various benefits over a centralized plan - it can better incorporate task context and allows LLMs to reason about individual robot capabilities. Additionally, natural language communication is interpretable and thus, allows the method to easily incorporate a human user to supervise or participate in the task. 
% This setup leverages both the world knowledge and emergent agentic capabilities \cite{nair2023dera} \footnote{\textcolor{red}{todo: add reference for this agentic point}} of LLMs: LLMs can reason about the semantics of a task and allocate resources among robots to efficiently distribute the work. Additionally, natural language communication is interpretable, and thus allows easy human supervision or intervention. This conversation-based channel also allows drop-in replacement of an agent with a human user, and the system can seamlessly work for both robot-robot and human-robot collaboration scenarios.  
 % Latest advancement in LLMs have demonstrated many skills beyond natural language, ranging across coding, tool use, mathematical reasoning, etc.

\textcolor{blue}{[GPT for path-planning]}
Next, we address the challenge of multi-robot motion planning by combining an LLM with a motion planner. In contrast to prior work that use LLMs for selecting action primitives, we explore the 3D spatial reasoning ability of an LLM and show that GPT-4 is surprisingly capable at 3D path planning purely from text and numerical coordinate inputs. When given the start, goal, and obstacle information, GPT-4 can plan collision-free paths for multiple agents. \footnote{\textcolor{red}{todo: I only used GPT4, need to confirm if GPT3/other LLMs can to this}} These waypoint paths then accelerate a motion planner by allowing it to sample the robots' joint space much more efficiently, and even succeed at planning otherwise infeasible trajectories. 
% LLM-planned waypoints naturally incorporate high-level semantics of a task, hence more efficient than hand-engineered waypoints specification. Good motion planning also benefits human-robot collaboration setups, where safety and fluency in robot motion is of utmost importance.  
 
% LLMs, deriving from their extensive pretrained data corpus, possess a rich source of task knowledge and conversational skills that would otherwise need to be separately designed \cite{cakmak2012designing}. Additionally, LLMs' in-context learning ability also enables generating personalize responses and actions based on individual human collaborators' preferences and needs. The pretrained models not only improve communication, but also provide context knowledge to robots for any task, enabling them to reason about human intentions and generate action plans effortlessly. Despite the lack of visual grounding in LLMs, recent state-of-the-art VLMs have been shown to generalize well on robotic task scenes \cite{zeng2022socratic,liang2022code}. For instance, open-vocabulary detection models have achieved high accuracy in detecting and localizing tabletop manipulation objects. Such VLMs translate environment observations into language descriptions, which can be fed into LLMs for reasoning and planning. Unlike prior work that requires a tailored system to fit the semantics of each task, pretrained models can be reused many times and are more adaptive to variations (such as different orders in a cooking recipe) than hand-coded task predicates. 

% HRC systems must prioritize minimizing safety risks while avoiding overly conservative behaviors that can hamper task efficiency. 
\textcolor{blue}{Improve plan by env. feedback}
Furthermore, we provide environment feedback to the LLM to further improve the path plan in-context. In cases where the zero-shot waypoint path is low-quality (i.e. cannot be used for motion planner), the environment computes the inverse kinematics (IK) and collision checking as feedback, and the LLM is prompted again to re-plan. We show that the LLM can correct the individual failed steps and improve the path. This feedback method is much relevant to recent work in tool-use \cite{yao2023react} and in-context feedback \cite{shinn2023reflexion}, where in our case it effectively lets an LLM better interact with the physical environment.

% Although numerous efforts have been made to address exemplifications of the aforementioned challenges in HRC, recent advances in machine learning offer potential for revolutionizing previous methodologies and alleviating the demand for engineering solutions. Some may argue that the involvement of humans in the collaboration process precludes the use of data-driven methods; however, recent paradigm shifts towards using web-scale pretrained models for domain-specific downstream tasks offer optimism for leveraging vision-language models in zero- or few-shot manners. The new state-of-the-art capabilities in visual perception and natural language processing ability of AI systems can be applied in a variety of applications in human-robot collaboration, which we explore in this work.
% \textcolor{blue}{\textbf{Maybe}: Sim-to-real transfer via learning vision-based policy}

% (Not sure about this part yet, my main question: 
% 1) Is sim-to-real transfer the only motivation for learning policy instead of motion planning? If we do things in sim., it doesn't seem to help in any way (given good waypoints proposed by GPT, motion plan is already very fast and precise). 
% 2) If answer to 1) is yes, instead of hoping a learned policy will transfer to real world, can we figure out a way to just directly motion plan in the real world, (or even map a sim env 1-to-1 directly to a real tabletop)? This seems more likely for transfer, and we can make a nice case for using env. feedback to let a GPT interact with the physical environment. 

\textcolor{blue}{[tl,dr our robot-robot, human-robot task env setup]}
We set up X tasks that require robot-robot human-robot collaboration use robots with different configuration and capabilities: both UR5E and Franka Panda arms, suction, and parallel-jaw grippers, etc. 

% 2. learning-based low-level control to execute the semantic action plans 
% The remaining challenge that vision or language models alone cannot solve is safe and fluent execution of robot motion. Accounting for the human's unpredictable and dynamic movements adds additional difficulty. This hinders motion planning techniques, which do well in static and fully observable states, and adjusting a robot's motion plan in real-time as the human moves or the environment changes makes it extra slow and inefficient. Another challenge is ensuring that the robot's motion is safe and legible for the human: beyond collision avoidance, factors such as the robot's speed and force when interacting with the human need to also be considered, to avoid causing harm or discomfort to the human. 
 

 \begin{figure}[t!]
     \centering
     \includegraphics[width=0.9\linewidth]{figures/fig1.001.jpeg}
     \caption{We leverage LLMs for high-level action and low-level motion planning, and demonstrate the effectiveness of this approach across a variety of multi-robot collaboration tasks.
     \shuran{in the figure, ideally, we highlight the range of tasks our system can do.  In the latter method figure we can explain how to do it. } 
     }
     \label{fig1}
 \end{figure}
 

\newpage 
\section{Multi-agent Planning via Conversational Prompting}
  \begin{figure}     
 \centering
     \includegraphics[width=0.99\linewidth]{figures/fig2.001.jpeg}
     \caption{
     % We use LLMs to plan both high- and low-level actions for collaborative tasks, provide environment feedback to improve the low-level path plans in-context, and then execute the final motion plan. 
     We study different prompting techniques for language-based robot communication: simulating agent chat versus a centralized plan.
     }
     \label{fig2}
 \end{figure}

